Information-Theoretic Bias Reduction via Causal View of Spurious Correlation

We propose an information-theoretic bias measurement technique through a causal interpretation of spurious correlation, which is effective to identify the feature-level algorithmic bias by taking advantage of conditional mutual information. Although several bias measurement methods have been proposed and widely investigated to achieve algorithmic fairness in various tasks such as face recognition, their accuracy- or logit-based metrics are susceptible to leading to trivial prediction score adjustment rather than fundamental bias reduction. Hence, we design a novel debiasing framework against the algorithmic bias, which incorporates a bias regularization loss derived by the proposed information-theoretic bias measurement approach. In addition, we present a simple yet effective unsupervised debiasing technique based on stochastic label noise, which does not require the explicit supervision of bias information. The proposed bias measurement and debiasing approaches are validated in diverse realistic scenarios through extensive experiments on multiple standard benchmarks.

==> sections/preliminaries.tex <==
% !TEX root = ../main.tex

\section{Preliminaries}
\label{sec:preliminaries} 




In this section we summarize CombCls~\cite{seo2019combinatorial} as this framework lies at the core of our approach. Then we analyze the characteristics of this methodology and discuss how it can be extended to the semi-supervised novel class retrieval problem.

\subsection{Combinatorial classification}
%\paragraph{Class codewords}

Unlike conventional classification approaches that directly predict the output class $y$, combinatorial classification~\cite{seo2019combinatorial} estimates $y \in \mathcal{C} = \{ 1, \dots, K\}$ by predicting its corresponding codeword.
The class codewords are constructed by defining $M$ meta-class sets, each of which is given by a unique partitioning of $\mathcal{C}$;
each meta-class set denoted by $\mathcal{C}^m$ ($m = 1, \dots, M$) has $K' (\ll K)$ meta-classes,~\ie~$\mathcal{C}^m= \{ c_{m, 1}, \dots, c_{m, K'} \}$, where multiple original classes are merged into a single meta-class; it results in attributes which describe discriminative properties shared among different classes.

Since the combinatorial classification framework predicts the class codewords to identify the class label $y$, $M$ individual classifiers, namely meta-classifiers, are constructed and each classifier estimates the conditional distribution $P(c^m_k|x)$ on a meta-class set $C^m$.
Each meta-classifier is trained by minimizing the sum of negative log-likelihoods of the ground-truth meta-class labels $\mathrm{meta}(y;m)$ that contain the ground-truth label $y \in \mathcal{C}$, \ie
%
\begin{equation}
     -\sum_{m=1}^M \log P(\mathrm{meta}(y;m)|x)
    \label{eq:sum_nll}
\end{equation}
%
The model will learn the relationship between input data and the semantic attributes. The model will use this learned relationship to recover the class label for inference input data.
To be specific, the conditional probability $P(y|x)$ on a original class set $C$ is reconstructed by combining the predictions of the learned meta-classifiers on meta-class sets as follows:
%
\begin{equation}
    P(c_k|x) = \frac{\prod_{m=1}^M{P\left(\mathrm{meta}(c_k ; m)\middle|x\right)}}{\sum_{j=1}^K\prod_{m=1}^M{P\left(\mathrm{meta}(c_j ; m)\middle|x\right)}}
    \label{eq:inference}
\end{equation}
%
\paragraph{\ghkim{[Extension to novel class identification]}}
The classification framework described above is fully supervised. However our goal is to aid the discovery of new classes by leveraging a certain number of known classes.
Note that, since CombCls can be interpreted as an attribute-based categorization, this procedure will even work for input data from a novel class if that class is included in the semantic knowledge base.
We can identify the characteristics of the samples from novel classes using their estimated codewords. Examples in novel classes may share some bits of the codewords with those in seen classes while having unique bits, which results in distinct codewords from the ones for the seen classes.




% \subsection{Applying to novel class identification}

% \paragraph{\ghkim{[Extension to novel class identification]}}
% We can apply the combinatorial classification for identifying novel classes.
% Since the partitioning strategy naturally introduces the inter-class relations into the model, a meta-class can be interpreted as an attribute representing a shared characteristic among its constituent classes, which become a basis of knowledge in labelled data to transfer for learning novel classes.

% Since combinatorial classification can be viewed as an attribute based categorization method, 
% we can identify the characteristics of the samples from novel classes using their codewords. 
% For instance, examples in novel classes may share some bits of the codewords with those in seen classes while having unique bits, which results in distinct codewords from the ones for the seen classes.
% Therefore, constituent classifiers can be easily extended to categorization models which consist of proxies for meta-classes and map each input to closest proxies.




%considered attribute shared between classes and convert classification problem into 
%to better generalization performance by learning meta-class representations from the examples in the multiple classes that %potentially have shared information.


